Slim NoC: A Low-Diameter On-Chip Network Topology for High Energy Efficiency and Scalability

Emerging chips with hundreds and thousands of cores require networks with unprecedented energy/area efficiency and scalability. To address this, we propose Slim NoC (SN): a new on-chip network design that delivers significant improvements in efficiency and scalability compared to the state-of-the-art. The key idea is to use two concepts from graph and number theory, degree-diameter graphs combined with non-prime finite fields, to enable the smallest number of ports for a given core count. SN is inspired by state-of-the-art off-chip topologies; it identifies and distills their advantages for NoC settings while solving several key issues that lead to significant overheads on-chip. SN provides NoC-specific layouts, which further enhance area/energy efficiency. We show how to augment SN with state-of-the-art router microarchitecture schemes such as Elastic Links, to make the network even more scalable and efficient. Our extensive experimental evaluations show that SN outperforms both traditional low-radix topologies (e.g., meshes and tori) and modern high-radix networks (e.g., various Flattened Butterflies) in area, latency, throughput, and static/dynamic power consumption for both synthetic and real workloads. SN provides a promising direction in scalable and energy-efficient NoC topologies.

==> abstract.tex <==
\begin{abstract}
%
Emerging chips with hundreds and thousands of cores require networks with
unprecedented energy/area efficiency and scalability. To address this, we
propose Slim NoC (SN): a new on-chip network design that delivers significant
improvements in efficiency and scalability compared to the state-of-the-art.
The key idea is to use two concepts from graph and number theory, 
degree-diameter graphs combined with non-prime finite fields, to enable the
smallest number of ports for a given core count. SN is inspired by state-of-the-art
off-chip topologies; it identifies and distills their advantages for NoC
settings while solving several key issues that lead to significant overheads
on-chip. SN provides NoC-specific layouts, which further enhance
area/energy efficiency. We show how to augment SN with state-of-the-art router
microarchitecture schemes such as Elastic Links, to make the network even more
scalable and efficient.  Our extensive experimental evaluations show that SN
outperforms both traditional low-radix topologies (e.g., meshes and tori) and modern
high-radix networks (e.g., various Flattened Butterflies) in
area, latency, throughput, and static/dynamic power consumption for both
synthetic and real workloads. SN provides a promising
direction in scalable and energy-efficient NoC topologies.
%
\end{abstract}

% \begin{abstract}
% %
% State-of-the-art datacenter and HPC topologies such as Dragonfly or Slim Fly
% are fast, inexpensive, and resilient. Thus, they are highly attractive on-chip
% network (NoC) candidates.
% %
% We first show that they unfortunately entail significant overheads when
% straightforwardly used as NoCs due to large buffers and long wires.  We then
% propose \tn\ (\TN): a diameter-2 NoC that resolves these problems.  \TN\ is
% inspired by Slim Fly and it uses graphs that approach \emph{radix-optimality}:
% they offer the fewest ports and thus buffer space for a given number of
% \hl{nodes}, also maximizing bandwidth.  Next, \TN\ offers NoC-specific layouts
% and placement models, further minimizing buffer area and power consumption.  We
% also show how to augment \TN\ with state-of-the-art microarchitecture schemes:
% Central Buffer routers, Elastic Links, ElastiStore, and SMART links,
% ensuring even more reductions in buffer space.
% %
% \TN\ outperforms both traditional low-radix topologies (meshes, tori) and
% modern high-radix networks (e.g., various Flattened Butterflies and
% hierarchical NoCs) in area, latency, throughput, and static/dynamic power
% consumption for both synthetic and real workloads.
% %
% The result is an energy-efficient, high-performance NoC capable of connecting a
% large number of cores in a scalable manner.
% %
% \end{abstract}

%
%
%
%
%\commt{Each ``CHANGE'' comment in the text describes what we changed in the
%paragraph below the respective comment.}
%
%\commt{We now provide a list of changes that occur in more than one section. We
%will not state them for each paragraph (unless there is some additional need to
%firmly underline something).}
%
%\commt{Color explanation: (1) \hlcyan{     CYAN     }: a paragraph was very heavily
%modified / improved, essentially a new one, (2) \hl{    APRICOT    }: a paragraph was
%strongly modified / improved, \hlgreen{    GREEN    }: a paragraph was moderately
%or cosmetically modified / improved.}
%
%\change{(1) We switch from the term ``endpoint'' and ``core'' to the term ''node''
%for a unified naming. We only use ``core'' if the context enforces or strongly
%  suggests it.}
%
%\change{(2) We ``decompress'' the text such that it is easier to read and follow. Specifically, the text was very dense
%in a way that a lot of information was packed in very little text or only in
%equations. After rewriting, basically every affected paragraph contains a lot
%more explanatory text. In addition, we have (a) improved the text grammatically, (b)
%and enhanced it in the ways it explains various ideas, concepts, etc.}
%
%\change{(3)
%We significantly reduce the use of symbols and abbreviations. Instead, we now use the full name
%of a given symbol as often as possible.}





